Generic Analysis of Model Product Lines via Constraint Lifting

Engineering a product-line is more than just describing a product-line: to be correct, every variant that can be generated must satisfy some constraints. To ensure that all such variants will be correct (e.g. well-typed) there are only two ways: either to check the variants of interest individually or to come up with a complex product-line analysis algorithm, specific to every constraint. In this paper, we address a generalization of this problem: we propose a mechanism that allows to check whether a constraint holds simultaneously for all variants which might be generated. The main contribution of this paper is a function that assumes constraints that shall be fulfilled by all variants and generates ("lifts") out of them constraints for the product-line. These lifted constraints can then be checked directly on a model product-line, thus simultaneously be verified for all variants. The lifting is formulated in a very general manner, which allows to make use of generic algorithms like SMT solving or theorem proving in a modular way. We show how to verify lifted constraints using SMT solving by automatically translating model product-lines and constraints. The applicability of the approach is demonstrated with an industrial case study, in which we apply our lifting to a domain specific modelling language for manufacturing planning. Finally, a runtime analysis shows scalability by analyzing different model product-lines with production planning data from the BMW Group and Miele.

==> text/sfit-impl.tex <==
\label{sec:sfit_smt}

After introducing the modeling language for the case study, we now show how we implemented our approach using the SMT solver Z3~\cite{de2008z3}.
Hereby, model product-lines and constraints are automatically translated to SMT to be analyzed. 
This translation itself is \emph{independent} of \sfit and translates arbitrary models of the Eclipse Modeling Framework (EMF) to SMT using the Z3 Java API. 

We use an illustrative \sfit model product-line that captures how a product-line of pens is manufactured. It can be seen in Figure~\ref{fig:sfit_model} and~\ref{fig:sfit_model_depl}. 
This model comprises parts and production steps for two variants of pens - one variant with a push button as opening mechanism; one variant with a twist mechanism.   
A feature model that captures this variability can be seen in the following SMT translation of a formula $\fModel_F$ of Section~\ref{sec:variability_mod} in SMT-LIBv2 syntax~\cite{cok2011smt}:

\begin{smt}{}
(declare-const PenFeatures bool) 
(declare-const OpenMechanism bool)
(declare-const TwistToOpen bool)  
(declare-const PushToOpen bool)

(assert (=> OpenMechanism PenFeatures))
(assert (=> OpenMechanism (or PushToOpen TwistToOpen)))
(assert (=> PushToOpen OpenMechanism))
(assert (=> TwistToOpen OpenMechanism))
(assert (=> TwistToOpen (not PushToOpen)))
(assert (=> PushToOpen (not TwistToOpen)))
(assert (=> PenFeatures OpenMechanism))
(assert (= PenFeatures true))
\end{smt}  

As one can see, Features are translated as uninterpreted bool constants. 
The feature tree structure and the \textit{requires} relation are expressed by the implications in lines 6 to 13.

Classes and objects are naturally translated as datatypes and datatype entities. 
Also the presence condition function $\config$ can be translated straight forward, as can be seen in the function \textit{selected\_part} for Part objects here:

\noindent\begin{minipage}{\linewidth}
\begin{smt}{}
(declare-datatypes ()(
  (Part BasePen PushButton TwistableHead NONE_Part)))
  
(declare-fun selected_part (Part) Bool)
(assert (= (selected_part BasePen) true))
(assert (= (selected_part PushButton) PushToOpen))
(assert (= (selected_part TwistableHead) TwistToOpen))
\end{smt}
\end{minipage}

Note, that for the datatype \textit{Part}, there also is an element \textit{NONE\_Part}. This corresponds to the usual notion of \textit{$\bot$} respectively \textit{null}.

Associations are formalized as functions in Section~\ref{sec:dsml}. 
They are also translated like this in SMT. 
The following SMT code results for the associations \textit{step} and \textit{machine} of class \textit{Deployment}:

\begin{smt}{}
(declare-fun Deployment_step (Deployment) ProductionStep)
(declare-fun Deployment_machine (Deployment) Machine)

(assert (= (Deployment_step Depl1) 
	(ite (selected_step PlaceBase) PlaceBase NONE_Step)))
(assert (= (Deployment_machine Depl1) GraspRobot))
(assert (= (Deployment_step Depl2) 
	(ite (selected_step InsertButton) InsertButton NONE_Step)))
(assert (= (Deployment_machine Deplt2) GraspRobot))
(assert (= (Deployment_step Depl3) 
	(ite (selected_step ScrewHead) ScrewHead NONE_Step)))
(assert (= (Deployment_machine Depl3) ScrewRobot))
\end{smt}

Here, one can also see the symbolic binding of variability using the SMT construct \textit{ite} (``if-then-else'') - just as in Definition~\ref{def:binding}.

Symbolic binding is also relevant for list associations. 
In SMT, we use \textit{sequences} and concatenation to form symbolic lists -- depending on the selection function, list members are translated either as one-element-sequences or empty sequences. 
With this, the list association \textit{parts} between the classes \textit{Product} and \textit{Part} results in:%\pagebreak
\begin{smt}{}
(declare-fun Prod_parts (Product) (Seq Part))

(assert (= (Prod_parts Pen) (seq.++
	(ite (selected_part BasePen) 
		(seq.unit BasePen) 
		(as seq.empty (Seq Part)))
	(ite (selected_part PushButton) 
		(seq.unit PushButton) 
		(as seq.empty (Seq Part)))
	(ite (selected_part TwistableHead) 
		(seq.unit TwistableHead) 
		(as seq.empty (Seq Part))))))
\end{smt}
Correctness constraints are already expressed in first order logic. 
We only need to negate them in order to let the SMT solver try to find one variant among all possible feature configurations that \emph{violates} the constraint.
Without this negation, the solver would search for \emph{one} feature configuration that fulfills all constraints instead of checking \emph{all} variants for one violation.
The constraint \textit{``All ProductionSteps are deployed to a Machine''} is lifted and translated:

\noindent\begin{minipage}{\linewidth}
\begin{smt}{}
(exists ((s ProductionStep)) 
	(and 
		(selected_step s) 
		(forall ((d Deployment)) (not(= (Deployment_step d) s)))))
\end{smt}
\end{minipage}

The constraint \textit{``For all Parts of all Products, there is a
ProductionStep that assembles the part''} is translated and lifted as:

\noindent\begin{minipage}{\linewidth}
\begin{smt}{}
(exists ((prod Product)) (exists ((p Part)) 
	(and 
		(seq.contains (Prod_parts prod)(seq.unit p)) 
		(selected_part p) 
		(forall ((s ProductionStep)) 
			(=> (and(selected_step s)) (not (= (Step_part s) p)))))))
\end{smt}
\end{minipage}


The third presented constraint \textit{``All ProductionSteps are deployed to a Machine that
can fulfill the ProductionStep's required Operation''} results in the following SMT expression:

\noindent\begin{minipage}{\linewidth}
\begin{smt}{}
(exists ((d Deployment)) (and 
(= 	(Operation_name (Step_required (Deployment_step d))) 
	(Operation_name	(Machine_provided (Deployment_machine d))))
(or 
	(> 
		(Operation_min (Step_required (Deployment_step d))) 
	 	(Operation_max (Machine_provided (Deployment_machine d)))) 
	(< 
		(Operation_max (Step_required (Deployment_step d))) 
	 	(Operation_min (Machine_provided (Deployment_machine d)))))
\end{smt}
\end{minipage}

This constraint shows that the lifting does not change navigation expressions -- even though \textit{(Step\_requiredOp(De- ployment\_step d))} navigates via potentially variable objects as \textit{ProductionStep}s.
This is correct, since the definition of the association \textit{Deployment\_step} above uses symbolic binding. 
Hence, it can only reach \textit{ProductionSteps} which are selected according to their presence condition.
